Self-supervised learning-based cervical cytology for the triage of HPV-positive women in resource-limited settings and low-data regime

Screening Papanicolaou test samples has proven to be highly effective in reducing cervical cancer-related mortality. However, the lack of trained cytopathologists hinders its widespread implementation in low-resource settings. Deep learning-based telecytology diagnosis emerges as an appealing alternative, but it requires the collection of large annotated training datasets, which is costly and time-consuming. In this paper, we demonstrate that the abundance of unlabeled images that can be extracted from Pap smear test whole slide images presents a fertile ground for self-supervised learning methods, yielding performance improvements relative to readily available pre-trained models for various downstream tasks. In particular, we propose \textbf{C}ervical \textbf{C}ell \textbf{C}opy-\textbf{P}asting ($\texttt{C}^{3}\texttt{P}$) as an effective augmentation method, which enables knowledge transfer from open-source and labeled single-cell datasets to unlabeled tiles. Not only does $\texttt{C}^{3}\texttt{P}$ outperforms naive transfer from single-cell images, but we also demonstrate its advantageous integration into multiple instance learning methods. Importantly, all our experiments are conducted on our introduced \textit{in-house} dataset comprising liquid-based cytology Pap smear images obtained using low-cost technologies. This aligns with our objective of leveraging deep learning-based telecytology for diagnosis in low-resource settings.

==> chapters/introductionDELETE.tex <==
\section{Introduction}
\label{sec:introduction_old}
Cervical cancer continues to be a major global health concern, with over 600,000 cases diagnosed and over 340,000 deaths reported worldwide in 2020 \cite{sung2021global}. The most significant burden of cervical cancer falls on settings that are least equipped to manage the disease, with the vast majority ($\sim$90\%) of cases affecting low-and middle-income countries (LMIC) \cite{gultekin2020world}. Periodic screening is known to significantly reduce the incidence and mortality of cervical cancer \cite{peto2004cervical}. It is predicted that adequate screening and treatment programs could prevent half of the predicted cervical cancer deaths over the next 50 years \cite{simms2019impact}. However, effective widespread screening is unobtainable in many countries, partly due to a lack of trained cytopathologists to diagnose Papanicolaou (PAP) tests. Moreover, producing cervical cytological slides is a labor-intensive and sometimes error-prone process \cite{elsheikh2013american,stoler2001interobserver}. Relying exclusively on human papillomavirus (HPV) testing is not a viable alternative diagnostic method due to its poor specificity, which results in overtreatment \cite{kuhn2020clinical}. The advent of digital microscopy and the recent evidence that digitally based diagnostic performance is on-par with light microscopy for Papanicolau test slides \cite{kholova2022inter} provides an interesting alternative. The added possibility of incorporating computer-assisted and/or automated diagnostics makes this an even more exciting prospect.\par
Histopathology-based assessment is considered the ``gold standard'' for most cancer-related diagnostics, and histology attracts far more attention from the machine learning community \cite{ABBET2022102473,stegmuller2023scorenet,bozorgtabar2021sood} than cytology. Recently though, cytopathology has gained more traction and recognition, as it offers a non-invasive and inexpensive diagnostic tool suited to resource-constrained countries. Consequently, there have been significant advancements in the field of machine learning applied to cytology. Most of these advancements focus on cell-level tasks, e.g., classification \cite{lin2019fine,albuquerque2021ordinal}, detection \cite{liang2021global,li2019detection} or segmentation \cite{hussain2020shape}. These innovations aim to improve the efficiency and accuracy of cervical cancer screening and other forms of cancer diagnosis from cytological samples.  \par
The classification of whole slide Pap smear images remains significantly less studied, despite being most promising in terms of its practical application. Notable works on the topic include \cite{cheng2021robust}, which combines low- and high-resolution stages for the identification/localization of suspicious lesions and their classification. The high-resolution stage relies on an RNN-based classification model to predict the WSI-level scores. Another study, \cite{wei2021efficient}, leverages a YOLO-based  \cite{redmon2018yolov3} approach to generate cell/tile-level predictions in the first stage, and a transformer model for the aggregation and WSI-level classification in the second stage. Similarly, \cite{cao2021novel} proposes to integrate an attention module to detect abnormal cells in large patches and compute the abnormality probability of a given patch as the average of its constituent cells. The WSI-level score is obtained by averaging the abnormality of its patches. \par
Cytology is only starting to attract machine learning practitioners, and, as such, there is relatively little literature on the subject. This work explores the possibilities and challenges of deep learning-based cytology diagnostics and systematically reports our findings. 
More precisely, we reveal the following facets of pap smear cytology:
\begin{itemize}
    \item We validate the usage of self-supervised pre-training to learn meaningful representations of cytology images for various downstream tasks. In particular, the resulting representations show superior discriminability and generalizability;
    \item Representations learned with publicly available single cervical cell datasets, e.g., Herlev \cite{jantzen2005pap}, or SIPAKMED \cite{8451588}, do not generalize well to different modalities such as images representing multiple cells;
    
    \item We experimentally show that we can learn generalizable representations from single-cell datasets with the appropriate data augmentation strategy;
    
    \item Multiple instance learning is the \textit{de facto} strategy to obtain WSI-level representations/predictions. Yet, it does not take full advantage of some inherent properties of pap smear cytology slides and is thus sub-optimal. We design a set of simple yet effective modifications to better benefit from the structure of the problem.
    \item \Thomas{We present a new dataset... }
\end{itemize}


==> tables/cells_to_tilesDELETE.tex <==
\begin{table}[ht]
\centering
\caption{
\Thomas{
\textbf{Transfer learning from Herlev and/or Sipakmed to our in-house labeled tiles dataset.} A k-NN classifier is fitted on the binary version of Herlev (H) and/or Sipakmed (S) datasets, and evaluated on the in-house set of positive cells/tiles. The features are extracted by a $\vit$-S/16 or a $\resnet$-50 pre-trained under a supervised pre-training on $\imagenet$ or a \hl{self-supervised pre-training} on our in-house unlabeled tiles dataset with DINO. The highest mean score for a given source dataset and backbone is indicated in \textbf{bold}.
}
}
\footnotesize
% \resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l c c c c}
\toprule
&&  \multicolumn{3}{c}{\textit{public cells $\rightarrow$ in-house tiles}}\\
\cmidrule{3-5}
\textit{backbone} && Herlev & Sipakmed  & Herlev + Sipakmed  \\ 
\midrule
$\resnet$-50                    &&  $52.9 \pm 6.3$ & $9.5 \pm 0.2$ & $14.0 \pm 4.3$\\
\rowcolor{cyan!20} $\resnet$-50 && $\mathbf{57.9 \pm 6.4}$ & $\mathbf{25.1 \pm 6.6}$ & $\mathbf{31.7 \pm 4.9}$\\
\midrule
$\vit$-S/16                    &&  $32.9 \pm 11.2$ & $5.3 \pm 2.6$ & $6.6 \pm 1.5$\\
\rowcolor{cyan!20} $\vit$-S/16 &&  $\mathbf{69.5 \pm 4.3}$ & $\mathbf{63.6 \pm 2.1}$ & $\mathbf{63.5 \pm 2.4}$\\
\bottomrule
\end{tabular}
% }
\label{table:cells_to_tiles}
\end{table}%


==> tables/knn_pasted_tilesDELETE.tex <==
\begin{table}[ht]
\centering
\caption{
\Thomas{
\textbf{Tiles-level evaluation of the frozen models} on a set of pasted tiles. A k-NN classifier is fitted on $75\%$ of the samples and evaluated on the remaining $25\%$. We report the class-wise and weighted $F_{1}$ scores of $4$ independent runs. The features are extracted by a $\vit$-S/16 or a $\resnet$-50 pre-trained under a supervised pre-training on ImageNet or a \hl{self-supervised pre-training} on our internal dataset with DINO. The highest mean score for a given class and backbone is indicated in \textbf{bold}.
}
}
\footnotesize
% \resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c}
\toprule
\textit{backbone} && positives & negatives & weighted $F_{1}$\\
\midrule
$\resnet$-50 && $81.3 \pm 2.2$  & $80.0 \pm 2.4$ & $80.7 \pm 2.2$ \\
\rowcolor{cyan!20} $\resnet$-50  && $\mathbf{82.1 \pm 1.6}$ & $\mathbf{81.8 \pm 1.5}$ & $\mathbf{82.0 \pm 1.6}$ \\
\bottomrule
$\vit$-S/16 && $73.5 \pm 1.3$ & $67.8 \pm 2.5$ & $70.7 \pm 1.8$ \\
\rowcolor{cyan!20} $\vit$-S/16 && $\mathbf{77.2 \pm 2.4}$ & $\mathbf{78.0 \pm 2.1}$ & $\mathbf{77.6 \pm 2.2}$ \\
\bottomrule
\end{tabular}
% }
\label{table:mixed_knn_tiles}
\end{table}%

==> tables/mil_newDELETE.tex <==
\begin{table*}[ht]
\label{table:mil}
\centering
\caption{
\Thomas{
We validate the different contributions of the proposed approach on a WSI classification task using a $\vit$ or $\resnet$ and common MIL methods.
}
}
\footnotesize
% \resizebox{0.85\columnwidth}{!}{
\begin{tabular}{l c c c c c c}
% \label{table:object_discovery}
\toprule
&& \multicolumn{2}{c}{WSI-level (AuC)} && \multicolumn{2}{c}{Tile-level (AuC)} \\ %&& \multicolumn{3}{c}{TokenCut \cite{wang2022self}}\\
\cmidrule{3-4} \cmidrule{6-7}
\textit{method} && $\vit$-S/16 & $\resnet$50 && $\vit$-S/16 & $\resnet$50 \\
\midrule
AbMIL~\cite{ilse2018attention} && $59.0 \pm 11.2$ & $61.1 \pm 11.2$ && $65.9 \pm 11.6$ & $61.6 \pm 12.5$ \\
+ Rand. Sampling                 && $65.5 \pm 10.4$ & $68.3 \pm 8.1$ && $64.3 \pm 10.4$ & $65.1 \pm 7.0$ \\
+ Top-K                          && $77.3 \pm 4.6$ & $64.4 \pm 8.4$ && $84.1 \pm 3.6$ & $75.3 \pm 10.9$  \\
+ Top-K + $\mathcal{L}_{loc}$    && $75.6 \pm 3.0$ & $77.2 \pm 2.6$ && $91.5 \pm 3.1$ & $89.8 \pm 2.1$ \\
\midrule
TransMIL~\cite{shao2021transmil} && $58.1 \pm 5.4$ & $49.9 \pm 5.2$ && $53.3 \pm 9.9$ & $46.7 \pm 10.7$ \\
+ Rand. Sampling                 && $63.4 \pm 7.0$ & $59.4 \pm 7.2$ && $50.9 \pm 12.4$ & $48.7 \pm 17.2$ \\
+ Top-K                          && $60.9 \pm 10.9$ & $60.0 \pm 9.7$ && $49.2 \pm 12.5$ & $56.0 \pm 19.8$ \\
+ Top-K + $\mathcal{L}_{loc}$    && $73.8 \pm 3.5$ & $77.3 \pm 5.2$ && $92.4 \pm 2.6$ & $93.1 \pm 2.0$ \\
\midrule
CLAM~\cite{lu2021data}         && $61.3 \pm 6.2$ & $64.3 \pm 11.1$ && $69.4 \pm 8.9$ & $61.4 \pm 11.3$ \\
+ Rand. Sampling                 && $61.2 \pm 6.2$ & $65.6 \pm 9.5$ && $68.9 \pm 6.7$ & $70.4 \pm 7.8$ \\
+ Top-K                          && $71.3 \pm 6.9$ & $65.3 \pm 12.4$ && $77.8 \pm 4.0$ & $70.4 \pm 10.2$ \\
+ Top-K + $\mathcal{L}_{loc}$    && $76.2 \pm 3.3$ & $79.5 \pm 5.6$ && $89.8 \pm 1.8$ & $91.4 \pm 2.4$ \\
\bottomrule
\end{tabular}
% }
\end{table*}%

==> tables/mixed_knn_cellsDELETE.tex <==
\begin{table*}[ht]
\centering
\caption{
\Thomas{
\textbf{Transfer learning from Herlev and/or Sipakmed to our in-house cells and tiles dataset.} A k-NN classifier is fitted on the binary version of Herlev (H) and/or Sipakmed (S) datasets, and evaluated on the in-house set of positive cells/tiles. The features are extracted by a $\vit$-S/16 or a $\resnet$-50 pre-trained under a supervised pre-training on ImageNet or a \hl{self-supervised pre-training} on our in-house unlabelled tiles dataset with DINO. The highest mean score for a given source dataset and backbone is indicated in \textbf{bold}.
}
}
\footnotesize
% \resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
&& \multicolumn{5}{c}{\textit{public cells $\rightarrow$ in-house cells}} && \multicolumn{5}{c}{\textit{public cells $\rightarrow$ in-house tiles}}\\
\cmidrule{3-7} \cmidrule{9-13}
\textit{backbone} && Herlev && Sipakmed  && Herlev + Sipakmed && Herlev && Sipakmed  && Herlev + Sipakmed \\ 
\midrule
$\resnet$-50                    && $\mathbf{94.8 \pm 0.9}$ && $70.0 \pm 4.2$ && $68.3 \pm 1.1$ && $52.9 \pm 6.3$ && $9.5 \pm 0.2$ && $14.0 \pm 4.3$\\
\rowcolor{cyan!20} $\resnet$-50 && $71.9 \pm 6.5$ && $\mathbf{84.0 \pm 4.0}$ && $\mathbf{82.1 \pm 3.8}$  && $\mathbf{57.9 \pm 6.4}$ && $\mathbf{25.1 \pm 6.6}$ && $\mathbf{31.7 \pm 4.9}$\\
\midrule
$\vit$-S/16                    && $\mathbf{93.4 \pm 1.7}$ && $59.7 \pm 3.5$ && $63.2 \pm 5.5$  && $32.9 \pm 11.2$ && $5.3 \pm 2.6$ && $6.6 \pm 1.5$\\
\rowcolor{cyan!20} $\vit$-S/16 && $84.1 \pm 2.3$ && $\mathbf{80.7 \pm 1.3}$ && $\mathbf{79.7 \pm 1.7}$  && $\mathbf{69.5 \pm 4.3}$ && $\mathbf{63.6 \pm 2.1}$ && $\mathbf{63.5 \pm 2.4}$\\
\bottomrule
\end{tabular}
% }
\label{table:mixed_knn_cells}
\end{table*}%


==> tables/mixed_knn_tilesDELETE.tex <==
\begin{table*}[ht]
\centering
\caption{
\Thomas{
\textbf{Tiles-level evaluation of the frozen models} on the in-house and pasted set of tiles. A k-NN classifier is fitted on $75\%$ of the samples and evaluated on the remaining $25\%$. We report the class-wise and weighted $F_{1}$ scores of $4$ independent runs. The features are extracted by a $\vit$-S/16 or a $\resnet$-50 pre-trained under a supervised pre-training on ImageNet or a \hl{self-supervised pre-training} on our internal dataset with DINO. The highest mean score for a given class and backbone is indicated in \textbf{bold}.
}
}
\footnotesize
% \resizebox{1.0\textwidth}{!}{
\begin{tabular}{l c c c c c c c c}
\toprule
&& \multicolumn{3}{c}{\textit{in-house tiles}} && \multicolumn{3}{c}{\textit{pasted tiles}} \\ 
\cmidrule{3-5} \cmidrule{7-9}
\textit{backbone} && positives & negatives & weighted $F_{1}$ && positives & negatives & weighted $F_{1}$\\
\midrule
$\resnet$-50 && $81.6 \pm 0.3$ & $79.1 \pm 0.5$ & $80.4 \pm 0.2$ && $81.3 \pm 2.2$  & $80.0 \pm 2.4$ & $80.7 \pm 2.2$ \\
\rowcolor{cyan!20} $\resnet$-50 && $\mathbf{95.3 \pm 0.6}$ & $\mathbf{95.1 \pm 0.7}$ & $\mathbf{95.2 \pm 0.6}$ && $\mathbf{82.1 \pm 1.6}$ & $\mathbf{81.8 \pm 1.5}$ & $\mathbf{82.0 \pm 1.6}$ \\
\bottomrule
$\vit$-S/16 && $77.8 \pm 0.6$ & $72.1 \pm 1.8$ & $74.9 \pm 1.0$ && $73.5 \pm 1.3$ & $67.8 \pm 2.5$ & $70.7 \pm 1.8$ \\
\rowcolor{cyan!20} $\vit$-S/16 && $\mathbf{96.6 \pm 0.4}$ & $\mathbf{96.4 \pm 0.5}$ & $\mathbf{96.5 \pm 0.4}$ && $\mathbf{77.2 \pm 2.4}$ & $\mathbf{78.0 \pm 2.1}$ & $\mathbf{77.6 \pm 2.2}$ \\
\bottomrule
\end{tabular}
% }
\label{table:mixed_knn_tiles}
\end{table*}%

